Soft X-ray AGN Luminosity Function from ROSAT Surveys II. Table of the binned Soft X-ray Luminosity Function

This is the second paper of our investigation of the 0.5-2 keV soft X-ray luminosity function (SXLF) of active galactic nuclei (AGN) using results from ROSAT surveys of various depth. The large dynamic range of the combined sample, from shallow large-area ROSAT All-Sky Survey (RASS)-based samples to the satellite's deepest pointed observation on the Lockman Hole, enabled us to trace the behavior of the SXLF. While the first paper (Miyaji, Hasinger, Schmidt 2000, hereafter paper I) emphasized the global behavior of the SXLF, cosmological evolution and contribution to the soft X-ray background, this paper presents actual numerical values for practical use of our results. To present the binned SXLF, we have used an improved estimator, which is free from biases associated with the conventional 1/Va estimator.

==> ReadMe <==

In this directory, we have included full ASCII Tables of the SXLF described 
in the paper. The ASCII tables contain columns which are not listed in 
corresponding Tables in the paper itself and the results for the 
'type I' sample are also included. Read Appendix A of paper I 
(Miyaji, Hasinger, Schmidt A&A, 353, 25) and for caveats when 
using the 'type I' sample. We did not include the z>1.6 bins in the 
'type I' sample because the values are identical to the all-AGN 
sample.

The ASCII Tables are:

cb3_f10_b1.exlf  : All AGNs          Omega_m=1.0, Omega_Lmabda=0.0  
cb3_f3_b1.exlf   :     "             Omega_m=0.3, Omega_Lmabda=0.7   
cb3_o3_b1.exlf   :     "             Omega_m=0.3, Omega_Lmabda=0.0   
cb3b_f10_b1.exlf : Type I sample     Omega_m=1.0, Omega_Lmabda=0.0  
cb3b_f3_b1.exlf  :     "             Omega_m=0.3, Omega_Lmabda=0.7   
cb3b_o3_b1.exlf  :     "             Omega_m=0.3, Omega_Lmabda=0.0   

Header/Footer/Comment lines begins with a "!". The columns are:

 zmin zmax zc: Redshift boundaries and central redshift of the bin.
 LgLmin Lmax Lc: Log L_x  boundaries and central Log L_x of the bin.
 Nobs: Number of AGNs in the bin
 Nmdl: Number of AGNs expected from the analytical model described in Sect 3.1.
 Phi^m: Analytical model evaluated at (z_c, L_c)
 Phi^n,er+,er-: SXLF value from the N^obs/N^mdl estimator and errors 
                 (Sect. 3.3)   
 Phi^v,er: SXLF value from the \sum 1/V_a etimator and error Sect. 3.2)

See the text of the paper for units of the SXLF values.

Takamitsu Miyaji (miyaji@astro.phys.cmu.edu) 












